Towards Anatomically Plausible Human Image Generation via Synthetic Localized Preferences

Large-scale text-to-image foundation models have achieved remarkable visual realism, yet generating human images with correct anatomical structures remains challenging. Existing approaches enforce anatomical constraints through part-specific modules or localized loss weighting during supervised fine-tuning on high-quality human photos, but such datasets are limited and often provide ambiguous optimization signals due to confounding factors such as lighting, pose, and background. Preference-based alignment offers an alternative, but standard Direct Preference Optimization (DPO) treats all pixels equally and therefore fails to exploit the localized nature of anatomical artifacts. To address this, we propose the framework of Alignment via Synthetic Anatomical Preference (ASAP), which constructs controlled preference pairs through a localized degradation mechanism applied to high-fidelity human images. This mechanism performs a controlled experiment on images by introducing explicit anatomical errors in targeted regions while preserving the remaining content. With this mechanism, we create the Human Anatomical Preference (HAP) dataset with over 10K curated pairs for effective anatomical alignment of text-to-image human image generative models. To better leverage the locality of these controlled preference pairs, we introduce a localized and margin-bounded variant of DPO that prioritizes optimization in targeted anatomical regions while enforcing a finite preference margin to prevent over-optimization and preserve global semantics. We further introduce HAF-Bench, a benchmark for systematic evaluation of anatomical fidelity. Extensive experiments demonstrate that ASAP consistently reduces anatomical errors across multiple foundation models while maintaining overall image quality.

==> figs/application.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% figs/application.tex — 单图应用示例（可选）
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%     \centering
%     \scriptsize
%     \begin{tikzpicture}
    % Placeholder figure: replace this tikzpicture with
    % \includegraphics[width=\linewidth]{pdfs/your_figure.pdf}
    \draw[line width=0.6pt, gray!60] (0,0) rectangle (12,3.5);
    \draw[gray!40] (0,0) grid[step=1] (12,3.5);
    \node[gray] at (6,1.75) {\scriptsize Figure placeholder};
\end{tikzpicture}
%     \caption{\scriptsize \textbf{Application of \modelname.} Placeholder.}
%     \label{fig:application}
% \end{figure}


==> figs/pipeline.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% figs/pipeline.tex — 方法总览图（通栏）
% 写法提示：
%   - 通栏图用 figure*，[t] 浮到页顶。
%   - 模板刻意不用 \vspace 手动微调间距（易造成图表重叠），
%     间距统一交给浮动体机制与 captionsetup 管理。
%   - caption 里用 \cref 串联各模块对应正文章节，图即目录。
%   - label 命名规范：fig:pipeline（fig: + 小写下划线）。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
    \centering
    \scriptsize
    \begin{tikzpicture}
    % Placeholder figure: replace this tikzpicture with
    % \includegraphics[width=\linewidth]{pdfs/your_figure.pdf}
    \draw[line width=0.6pt, gray!60] (0,0) rectangle (12,3.5);
    \draw[gray!40] (0,0) grid[step=1] (12,3.5);
    \node[gray] at (6,1.75) {\scriptsize Figure placeholder};
\end{tikzpicture}
     \caption{\scriptsize \textbf{Pipeline of \modelname.} Placeholder: given
     input \refimg, we first ... ~(\cref{sec:method_a}), then generate ...
     with module B~(\cref{sec:method_b}), and finally reconstruct ...
     ~(\cref{sec:method_c}).}
    \label{fig:pipeline}
\end{figure*}


==> figs/qualitative.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% figs/qualitative.tex — 双图并排示例（minipage 版 "subfigure"）
% 说明：本模板不用 subcaption/subfigure 宏包，并排小图用两个 minipage
%       手工组合（0.60 + 0.36 textwidth，中间 \quad），各自带独立 caption
%       与 label。这是组内惯用做法，浮动体控制更直接。
%       注意：TikZ 占位图宽度按 minipage 宽度适配（左 7.5cm / 右 4.5cm）。
% 若需要正式的 子图编号，可启用 subcaption：在 config/package.tex 加
%   \usepackage{subcaption}，然后：
%   \begin{subfigure}{0.48\textwidth} ... \subcaption{...} \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \scriptsize
    \begin{minipage}[t]{0.60\textwidth}
    \begin{tikzpicture}
    % Placeholder figure: replace this tikzpicture with
    % \includegraphics[width=\linewidth]{pdfs/your_figure.pdf}
    \draw[line width=0.6pt, gray!60] (0,0) rectangle (7.5,2.5);
    \draw[gray!40] (0,0) grid[step=1] (7.5,2.5);
    \node[gray] at (3.75,1.25) {\scriptsize Figure placeholder};
\end{tikzpicture}
    \caption{\scriptsize{\textbf{Qualitative Comparisons.}}}
    \label{fig:qualitative}
    \end{minipage}
    \quad
    \begin{minipage}[t]{0.36\textwidth}
    \begin{tikzpicture}
    % Placeholder figure: replace this tikzpicture with
    % \includegraphics[width=\linewidth]{pdfs/your_figure.pdf}
    \draw[line width=0.6pt, gray!60] (0,0) rectangle (4.5,2.5);
    \draw[gray!40] (0,0) grid[step=1] (4.5,2.5);
    \node[gray] at (2.25,1.25) {\scriptsize Figure placeholder};
\end{tikzpicture}
    \caption{\scriptsize \textbf{Zoom-in Comparison.}}
    \label{fig:qualitative_zoom}
\end{minipage}
\end{figure}


==> sec/6_applications.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sec/6_applications.tex — 应用展示（可选节）
% 写法提示：
%   - 展示方法带飞的下游任务（try-on、animation、editing 等），一图一事。
%   - 页数紧张时整节移到附录，正文 conclusion 前一句话指路。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Applications}
\label{sec:applications}

Placeholder: \modelname enables downstream task X for free, as shown
in~\cref{fig:teaser}. More examples in~\suppl's~\cref{sec:supl_app}.


==> sec/7_limitation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sec/7_limitation.tex — 局限与展望（可选节）
% 写法提示：
%   - ICLR 2026 起正文页数紧张，组内惯常做法：本节内容并入附录
%     x_appendix.tex（sec:supl_limitation），正文 conclusion 一句话指路。
%   - 如确需在正文出现，取消 main.tex 中对应 \input 的注释即可。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Limitations and Future Work}
\label{sec:limitation}

Placeholder: limitations are discussed in~\suppl's~\cref{sec:supl_limitation}.


==> tabs/ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tabs/ablation.tex — 消融表
% 写法提示：
%   - 每行一个变体，勾叉列用 \cmark / \xmark（notation.tex）。
%   - 最优配置行 \rowcolor{gray!20}。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|cc|cc}
\bottomrule
Variant & \cmark{} Component A & \cmark{} Component B & \down{Chamfer$\downarrow$} & \up{PSNR$\uparrow$} \\ \cline{1-5}
Baseline     &          &          & 0.000  & 0.00  \\
+ A          & \cmark  &          & 0.000  & 0.00  \\
+ B          &          & \cmark  & 0.000  & 0.00  \\ \rowcolor{gray!20}
Full (\modelname) & \cmark & \cmark & \textbf{0.000} & \textbf{0.00} \\ \toprule
\end{tabular}}
\caption{\textbf{Ablation Studies.} Placeholder: each row enables one component.}
\label{tab:ablation}
\end{table}


==> tabs/quantitative.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tabs/quantitative.tex — 主结果表
% 组内表格规范（源自 2026 版）：
%   1. 三线表变体：底部 \bottomrule 在表头行、顶部 \toprule 在末行
%      （本表头在上、数据在下、倒置三线风格，视觉上更轻）。
%   2. 指标方向：\up{PSNR$\uparrow$} / \down{LPIPS$\downarrow$}
%      表头即带绿/红底色（定义在 config/preamble.tex）。
%   3. 最优行高亮：\rowcolor{gray!20} 放在数据行前。
%   4. 多数据集分组：\multicolumn{6}{c|}{DatasetA} + \cline{2-15}。
%   5. \resizebox{\textwidth}{!}{...} 压缩超宽表格；行距 \arraystretch=1.2。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\bottomrule
             & \multicolumn{3}{c|}{Dataset A} & \multicolumn{3}{c}{Dataset B}  \\ \cline{2-7}
             & \up{PSNR$\uparrow$}   & \up{SSIM$\uparrow$}   & \down{LPIPS$\downarrow$}  & \up{PSNR$\uparrow$}   & \up{SSIM$\uparrow$}   & \down{LPIPS$\downarrow$}   \\ \cline{1-7}
Baseline 1   &   00.00         &   0.000          &  0.000           &  00.00        &   0.00        &    0.000            \\
Baseline 2   &   00.00         &   0.000          &  0.000           &  00.00        &   0.00        &    0.000            \\ \rowcolor{gray!20}
Ours         & \textbf{00.00}  & \textbf{0.000}   & \textbf{0.000}   & \textbf{00.00} & \textbf{0.00} & \textbf{0.000}    \\ \toprule
\end{tabular}}
\caption{\textbf{Quantitative Comparison with Baselines.} Placeholder:
\modelname achieves the best ... on Dataset A and B.}
\label{tab:quantitative}
\end{table}

